DPFM: Deep Partial Functional Maps

We consider the problem of computing dense correspondences between non-rigid shapes with potentially significant partiality. Existing formulations tackle this problem through heavy manifold optimization in the spectral domain, given hand-crafted shape descriptors. In this paper, we propose the first learning method aimed directly at partial non-rigid shape correspondence. Our approach uses the functional map framework, can be trained in a supervised or unsupervised manner, and learns descriptors directly from the data, thus both improving robustness and accuracy in challenging cases. Furthermore, unlike existing techniques, our method is also applicable to partial-to-partial non-rigid matching, in which the common regions on both shapes are unknown a priori. We demonstrate that the resulting method is data-efficient, and achieves state-of-the-art results on several benchmark datasets. Our code and data can be found online: https://github.com/pvnieo/DPFM

==> sec-experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Baselines}
% %In the following, we  denote our method as \textit{Ours}, and compare it to a wide spectrum of partial shape matching methods, both axiomatic and learning-based ones. For the axiomatic methods, we compare to PFM \cite{Rodol2016}, FSP \cite{Litany2017}, DOC \cite{Cosmo2016} and a very recent Dual Iterative Refinement Method (DIR) \cite{Xiang_2021_CVPR} that has been shown to outperform several other existing baselines. As there is no previous work treating non-rigid partial shape matching in a learning setting, we used GeomFMaps as our learning baseline, as it is the closest to our design. Except for DIR, which is itself a refinement method, we also apply ZoomOut adapted to partiality \cite{Melzi2019} to all the other methods, and report results with and without refinement. 

% %For all the competing methods, we used the original code released by the authors, and the best parameters reported in the paper and code.
We compare with the following prior partial shape matching methods: PFM \cite{Rodol2016}, FSP \cite{Litany2017}, DOC \cite{Cosmo2016} and also very recent Dual Iterative Refinement Method (DIR) \cite{Xiang_2021_CVPR}. Since this work is the first to tackle a \emph{learning} approach to non-rigid partial shape matching, we also include GeomFMaps \cite{Donati2020} as a learning baseline, since this is similar in spirit to our method. In addition, we refine almost all methods with the partial variant of the Zoomout algorithm \cite{Melzi2019}. For all  competing methods, we use the original code released by the authors and apply the best parameters reported in the respective papers.

\section{Experiments and Analysis}
\label{sec:experiments}
In this section, we provide extensive experiments highlighting the accuracy and robustness of our method, on a range of non-rigid partial shape matching tasks. We consider three main tasks: partial-to-full, partial-to-partial, and finally partial-to-full under extreme mesh variability. To this end, we use, on one hand, the available partial benchmarks, and on the other hand, introduce two datasets for two new tasks. %We provide both quantitative and qualitative results.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure*}[h]
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{figures/princeton_cuts}
%   \caption{Cuts subsets}
%   \label{fig:princeton_p2f_cuts}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{figures/princeton_holes}
%   \caption{Holes subsets}
%   \label{fig:princeton_p2f_holes}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Correspondence quality of different methods on the test set of SHREC'16 Partial Benchmark, both on cuts (left) and holes (right). Our method shown in red, outperforms all the competing methods, and achieves state of the art results. Mean errors of all methods are reported in the legend.\vspace{-4.5mm}}
% \label{fig:princeton_p2f}
% \end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Datasets}
\label{sec:datasets_prez}
In order to evaluate our method both quantitatively and qualitatively, we use a wide spectrum of non-rigid partial benchmarks.

\textbf{The SHREC'16 Partial Correspondence Benchmark \cite{cosmo2016shrec}} is the standard dataset to evaluate partial non-rigid matching methods. This dataset consists of 76 nearly isometric shapes, divided into 8 classes (humans and animals). Each class has a 'null' shape in a neutral position, to which the partial shapes will be matched. These  shapes are individually re-meshed to 10K vertices for an additional challenge. 

Two partial subsets are constructed based on this dataset, namely \textbf{CUTS} and \textbf{HOLES}. \textbf{CUTS} is constructed by cutting the shapes with a random plane at different orientations. \textbf{HOLES} is more challenging since the shape's surfaces have been eroded starting from some random seeds over the surface, causing them to have holes and irregular cuts.

\textbf{SHREC'16 Part-to-Part dataset (\textbf{CP2P})}: We introduce this dataset, which we created based on the \textbf{CUTS} training set in  \cite{cosmo2016shrec}, resulting in 120 different partial shapes and over 300 pairs. Our dataset contains the same 8 classes of humans and animals in different poses and partialities, and it presents the challenge that only part of the source shape is mapped to only a part of the target shape. The overlap between the source and target can range from 10\% to 90\% of the total area. The train and test sets are divided randomly so that 80\% of pairs are used for training, and the remaining 20\% are used for testing. It should be noted, that similar to \textbf{CUTS} and \textbf{HOLES}, the ground truth map is only provided for shapes from the same class.

\textbf{Partial FARM dataset (\textbf{PFARM})}: As many shape matching pipelines are known to overfit the mesh connectivity, we introduce another dataset to test the robustness of the different methods on shapes that undergoes non-isometric deformations with significantly different connectivity. This dataset is based on shapes from the SHREC'19 track \cite{shrec19connectivity}, and can be considered as an extension to the recently introduced FARM partial dataset \cite{Kirgo2020}, but with more test shapes. This dataset is composed of 27 test pairs and 28 different human shapes that have different meshing and vertex density, and undergo rigid and non-rigid deformations, in addition to the partiality introduced by cutting random patches in each shape. Some example shapes of all the previous datasets are provided in the supplementary. 

\mypara{Evaluation Protocol}
We follow the Princeton protocol \cite{Kim2011} to evaluate all correspondences, as used in all recent works. Namely, we compute the geodesic errors for all the predicted maps with regard to the given ground truth map and normalize the scale by the square root of the total surface area of the target shape.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Part To Full Shape Matching}
\label{subsec:p2f_exp}
We first test our method on the task of partial-to-full matching using \textbf{CUTS} and \textbf{HOLES} datasets. We train our networks separately on the train set of each dataset composed of 120 and 80 pairs consecutively. In addition, we train our sparse variant Ours$_{\text{sparse}}$ on the HOLES dataset, as the latter can handle particularly sparse data, and show that our architecture is not limited to the choice of the feature extractor. 

It should be noted that contrary to many of the previous works, which are evaluated on the train set of \textbf{CUTS} and \textbf{HOLES}, we follow the original SHREC'16  Benchmark protocol, and test our method, and all the baselines \emph{only on the test set}, which contains 200 pairs each for \textbf{CUTS} and \textbf{HOLES}. The test set contains unseen shapes during training and provides a diverse and \emph{significantly} more challenging set of partiality scenarios.

As reported in Figure \ref{fig:princeton_p2f} and in the supplementary materials, our method achieves state-of-the-art results across all settings, on both the cuts and holes datasets, outperforming both axiomatic and learning-based methods. In addition, we evaluate the behavior of our method with an increasing amount of partiality, measured as a percentage of the missing area. It can be seen from the plots reported in the supplementary materials that our method achieves the lowest mean geodesic error among all methods, and the error stays nearly constant as the amount of partiality increases, which shows the robustness of our method. Last but not least, as our method can also predict the overlap region, which is a feature of only PFM, we evaluate the quality of the latter by computing the intersection over union (IOU) of the predicted region and the ground truth one. It can be seen from the figure in the supplementary materials that our method achieves a high IOU, outperforming PFM, especially for the cuts dataset, which demonstrates the quality of the predictions made by the overlap module. Finally, We provide qualitative illustrations of the resulting correspondences in the supplementary material on a range of test pairs.


% \begin{figure*}[h]
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{figures/princeton_cuts}
%   \caption{Cuts subsets}
%   \label{fig:princeton_p2f_cuts}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{figures/princeton_holes}
%   \caption{Holes subsets}
%   \label{fig:princeton_p2f_holes}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Correspondence quality of different methods on the test set of SHREC'16 Partial Benchmark, both on cuts (left) and holes (right). Our method shown in red, outperforms all the competing methods, and achieves state of the art results. Mean errors of all methods are reported in the legend.\vspace{-4.5mm}}
% \label{fig:princeton_p2f}
% \end{figure*}

\begin{figure}[]
\begin{center}
\includegraphics[width=\linewidth]{figures/princeton_cuts}
\end{center}
\vspace{-2mm}
  \caption{Correspondence quality of different methods on the \textbf{CUTS} test set of SHREC'16 Partial Benchmark (\textbf{HOLES} is provided in the supplementary materials). Our method shown in blue outperforms all the competing methods and achieves state-of-the-art results. Mean errors of all methods are reported in the legend.\vspace{-4.5mm}}
\label{fig:princeton_p2f}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Robust Part To Full Shape Matching}
\label{subsec:robust_p2f_exp}
As was shown in previous works \cite{Donati2020}, methods relying on handcrafted features, such as SHOT, tend to overfit  the mesh connectivity and endure a huge performance drop when they are faced with meshes with different connectivity. To test this in the partial setting, we perform an evaluation of all the baselines on the \textbf{PFARM} dataset. As the size of this dataset is small and is not adapted to training, we only used the pre-trained networks on CUTS for both our method and GeomFMaps. 

The Princeton benchmark results are provided in Figure \ref{fig:princeton_farm}. Our method achieves the best result among all the baselines. Also, as expected, traditional methods relying on hand-crafted features endured a huge drop in performance, this is in contrast with learning-based methods that do not overfit to the mesh connectivity, and still perform better, even in the case of using a pre-trained network. Finally, qualitative results are shown in Figure \ref{fig:quali_farm}. It can be seen that only our method yields visually plausible correspondence.


\begin{figure}[]
\begin{center}
\includegraphics[width=0.9\linewidth]{figures/princeton_pfarm}
\end{center}
\vspace{-2mm}
   \caption{Results on the PFARM dataset. Our method is  robust to significant changes in mesh discretization, and outperforms all the baselines, whether learning-based or axiomatic. \vspace{-1mm}}
\label{fig:princeton_farm}
\end{figure}

\begin{figure}[]
\begin{center}
\includegraphics[width=1\linewidth]{figures/pfarm_texture_transfert}
\end{center}
\vspace{-3mm}
  \caption{Qualitative results on the FARM Partial dataset using texture transfer. Only our method produces visually plausible results.\vspace{-6mm}}
\label{fig:quali_farm}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Part To Part Shape Matching}
\label{subsec:p2p_exp}
We also evaluate our method on the challenging task of partial-to-partial shape matching, where only a portion of the source shape is mapped to a portion of the target shape. We compare our method against PFM, the formulation of FSP adapted to this setting, the learning-based baseline GeomFMaps, and DOC, the method outlined in \cite{Cosmo2016}. We use the new dataset \textbf{CP2P} for this purpose, and the evaluation is performed in two ways. First, the mean geodesic error is evaluated only on the overlap region, resulting in a Princeton graph, and second, the IOU of the predicted overlap region is evaluated to measure the region detection ability. %However, only our method produces an overlap region in this setting. 
We apply the PFM method in both directions (source to target and target to source), thereby generating a predicted region of overlap on both source and target shapes. Since DOC \cite{Cosmo2016} already optimizes for two overlap regions, we use their method as-is by initializing with SHOT descriptors. 

The Princeton benchmark in Figure \ref{fig:princeton_p2p} shows the superiority of our method over the baselines. Also, even if FSP was tailored for this setting, it still gives a lower result than two-way PFM. Finally, we get better region prediction as shown in the IOU figure reported in the supplementary.



\begin{figure}[]
\begin{center}
\includegraphics[width=0.9\linewidth]{figures/princeton_p2ph}
\end{center}
\vspace{-3mm}
   \caption{Quantitative results of the different methods on the CP2P dataset. Our method achieves superior results, outperforming all  baselines.  \vspace{-3mm}}
\label{fig:princeton_p2p}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypara{Ablation Study}
Our architecture is composed of multiple building blocks that we consider essential for optimal performance. To validate this, an ablation study is performed in the supplementary materials.

% \paragraph{Mask Ablation}
% \begin{table}
% \begin{center}
% \begin{tabular}{|l|c|c|c|}
% \hline
% \textbf{Mask} & \textbf{Laplacian Mask} & \textbf{Slanted Mask} & \textbf{Our Mask} \\
% \hline\hline
% CUTS & 3.5 & 4.27 & \textbf{3.2} \\
% \hline
% HOLES & 14.6 & 14.5 & \textbf{13.1} \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Ablation of Masks}
% \label{table:mask}
% \end{table}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Loss Ablation}

% \begin{table}
% \begin{center}
% \begin{tabular}{cc}
% \hline
% \textbf{Ablation} & \textbf{Mean Error on HOLES}\\
% \hline
% no spectral loss & 32 \\
% no NCE loss & 14.6 \\
% no Refinement Block & 13.8 \\
% Total loss & \textbf{13.1}\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Ablation of losses}
% \label{table:loss_abla}
% \end{table}


